Stable Matching with Interviews

In several two-sided markets, including labor and dating, agents typically have limited information about their preferences prior to mutual interactions. This issue can result in matching frictions, as arising in the labor market for medical residencies, where high application rates are followed by a large number of interviews. Yet, the extensive literature on two-sided matching primarily focuses on models where agents know their preferences, leaving the interactions necessary for preference discovery largely overlooked. This paper studies this problem using an algorithmic approach, extending Gale-Shapley's deferred acceptance to this context. Two algorithms are proposed. The first is an adaptive algorithm that expands upon Gale-Shapley's deferred acceptance by incorporating interviews between applicants and positions. Similar to deferred acceptance, one side sequentially proposes to the other. However, the order of proposals is carefully chosen to ensure an interim stable matching is found. Furthermore, with high probability, the number of interviews conducted by each applicant or position is limited to $O(\log^2 n)$. In many seasonal markets, interactions occur more simultaneously, consisting of an initial interview phase followed by a clearing stage. We present a non-adaptive algorithm for generating a single stage set of in tiered random markets. The algorithm finds an interim stable matching in such markets while assigning no more than $O(\log^3 n)$ interviews to each applicant or position.

==> proposal.tex <==

\section{Proposal}

Many two-sided markets, such as labor and dating markets, involve agents who have incomplete information about their preferences before they interact with one another. For example, in the medical labor market, residency and fellowship candidates often apply to multiple programs to increase their chances of securing interviews and finding good matches. Virtual interviews have made it cheaper and easier for candidates to interview with more programs, but this has also led to increased congestion in the interviewing process \cite{hammoud2020improving}. To address the steady increase in the number of interviews, some have proposed limiting the number of applications that agents can make and allowing agents to signal their interests to a limited number of firms. However, these solutions may not necessarily reduce the number of interviews or the cost to reviewing applications.  A partial solution uses signaling \cite{coles2010job} of preferences and the  PI  Ashlagi proposes the need for an  interview match \cite{melcher2019may, melcher2019reducing}  for residencies and fellowships. In this proposal, we set up a basic model and study the  algorithmic foundations for this challenge that involves matching and communicating information. 

%In many two-sided markets, such as labor markets and online dating, agents often have only partial information about their preferences before they meet. For example, in the medical labor market, residency and fellowship candidates often apply to multiple programs in order to increase their chances of securing interviews and matching favorably. The use of virtual interviews has reduced the costs and increased the number of interviews. The steady increase in the number of interviews is an example of a congestion re is a need to find ways to increase the efficiency of applications and interviews and reduce the congestion in the interviewing process. Some proposals have suggested capping applications and allowing agents to signal their interests to a limited number of firms, but these solutions may not necessarily limit the number of interviews.

%In many two-sided  markets, agents have only partial information about their preferences before they actually meet. In labor markets this typically involves  interviews, in online dating this means exploring ones profile or meeting on a date. In  medical labor markets for residency  and fellowship candidates are applying to more programs to enhance their chances of securing interviews and matching favorably. Virtual interviews have reduced some costs, especially for candidates, but increased the number of interviews.  Several proposals suggest ways to increase the efficiency of applications and interviews. The number of interviews is steadily increasing, and there is need to ease congestion in this interviewing process. Different approaches have been proposed such as capping applications and allowing agents to signal their interests to few firms beyond the regular applications. These solutions, however, may not bound the number of interviews.   

 

We extend the classic two-sided marriage problem to the case where the agents  only partially know their own preferences, and only after ``meeting" a partner they find out how much they like them. Suppose there are $n$ applicants interested in $n$ positions. The utility of position $j$ for applicant $i$ can be written $v_j + \epsilon_{ij}$. The quantity $v_j$ reflects the characteristics of the position, like working hours, salary, or prestige, and is public knowledge. $\epsilon_{ij}$ reflects applicant $i$'s subjective interest in position $j$, which will only be revealed to the applicant after the interview. We assume  $\epsilon_{ij}$'s are independently sampled from a known distribution with mean zero. Define the utility of position $j$ in applicant $i$ as $u_i + \epsilon_{ji}$ similarly. 

We  define interim stable matchings.  Let the {\em observed utility} of $i$ in $j$, $u^o_{ij}$ be $v_j + \epsilon_{ij}$ if $i$ and $j$ have interviewed, and equal to $v_j$ otherwise. Define $v^o_{ji}$'s or the observed utility of positions in the applicants similarly. A matching $M$ is interim stable if all the matched pairs have interviewed with each other and there are no blocking pairs with respect to observed utilities, i.e., $\{i, j\} \in M$ and $\{k, l\} \in M$ imply either $v^o_{ji} \geq v^o_{jk}$ or $u^o_{kl} \geq u^o_{kj}$. 

Our recent preliminary result  gives a polynomial-time algorithm that finds an interim stable matching with only a  near-linear number of interviews. 
\begin{theorem}
   It is possible to find a stable matching with respect to observed utilities in polynomial time and with at most $O(n\log n)$ interviews in expectation.
\end{theorem}

We can also show that with high probability, the algorithm will not ask any applicant or position to do more than $O(\log^2 n)$ interviews. 
The algorithm is an extension of the Gale-Shapley mechanism in which the order of interviews is chosen carefully and adaptively. The proof uses a potential function and an exposure martingale's analysis. Several open problems remain: 

\begin{itemize}
    \item Our algorithm proposes the sequence of interviews adaptively, suggesting each interview based on the outcome of the earlier ones. On the other hand, many markets have a more simultaneous flavor, in which there is a stage of interviews followed by a clearing phase. As a result, it is more desirable for the interview lists to be decided either in advance or for each position independently from others. Is there an algorithm that comes up with the interview lists in one round or a small number of rounds? 
 
    \item The above formulation assumes a universal ranking of applicants and positions before  interviews. That may be too restrictive. A natural extension is to divide the utility functions into three parts, i.e., $v_j+\delta_{ij}+\epsilon_{ij}$,  where $v_j$ reflects the global ranking of the position, $\delta_{ij}$, the subjective preference of applicant $i$ in position $j$, and $\epsilon_{ij}$, the information gained from the interview. 
    
    \item We are also interested in the fairness of the above stability notion and our proposed algorithms, especially in scenarios where the distribution of $\epsilon_{ij}'s$ are different from each other. What is the tradeoff between the number of interviews and the fairness of the process? Formulating the notion of fairness and developing fair algorithms is an interesting open direction. 
\end{itemize}



In order to answer the first question, 
we study matching algorithms that work in two phases. In the first phase, the algorithm generates a list of interviews with relatively ``few" interviews for each agent. After each interview, the agent and the position observe their utilities for each other. In the second phase, the agent-proposing deferred acceptance algorithm generates the final one-to-one matching, with agents ranking only partners from their interview set and the preferences induced by the actual utilities for their interviews. 


One natural candidate for the first phase of the algorithm that generates the interview list is the many-to-many  variation of the deferred acceptance in which each applicant and position has a capacity of $k$. We aim to determine the optimal value of $k$ needed for agents to achieve a high enough match rate and asymptotic interim stability in which a vanishing number of agents are left in blocking pairs and do not regret their decision to interview. 
We also want to investigate whether it is possible to design an incentive-compatible interview matching mechanism that would allow agents to reveal their preferences over potential partners to the mechanism.

In preliminary results, we find structural assumptions under which this is possible. Our work builds on an extension of the model in which  the priority utility of agent $i$ for position $j$ is $v_j+\delta_{ij}$ and the actual (ex-post) utility is $v_j+\delta_{ij}+\epsilon_{ij}$. Similarly each position $j$ for agent $i$ has utility $u_i+\delta_{ji}+\epsilon_{ji}$. While the $v_j$'s and $u_i$'s are known, the additional apriori tastes $\delta$'s can be private information.  
\begin{theorem}
   Let $n$ be the number of agents on each side and assume that $u_i$'s, $v_j$'s,  $\delta_{ij}$'s, $\delta_{ji}$'s are generated from $U[0,1]$ (or any bounded and continuous distribution). Further, assume that the post-interview $\epsilon$'s are generated from $U[-1,1]$. Then the many-to-many deferred acceptance algorithm with interview capacity $k\geq 2$ on each side has the following properties as $n\to\infty$.
   \begin{itemize}
   \item The match rate converges to at least $1 - e^{-\sqrt{k}}$ and pre-interview match qualities converge to $1$.
    \item\ Post-interview match quality for hospitals and post-interview match quality for doctors are bounded from below by   $1 - \frac{2}{\sqrt{k}}.$
    \item\label{thm-main-stability}  The fraction of positions that in blocking pairs are at most $2^{-\sqrt{k}}.$
    \item  For any  $n$ sufficiently large, it is an $\gamma$-Bayes Nash equilibrium where with high probability every agent reports their preferences truthfully, for $\gamma\geq e^{-\sqrt{k}}.$
   \end{itemize}
\end{theorem}


Intuitively, as the market grows larger, each agent interviews  agents of roughly the same quality. The proof relies  on analyzing the random proportional random graph generated from  these a-priori utilities and bounding the relevant measures. Note that the interview graphs are not cliques due to the apriori tastes. 
%;  That  $k$ is similar for each agent is required not only for the match rages but also for incentive compatibility.  


We plan to  extend these results to allow for less restrictive assumptions on the market structure, such as allowing more tiers. In such markets, one may need to assure the competitive structure of the market is not altered in order to both achieve stability and incentive compatibility. We are interested in how many ``rounds" of communication are needed to reach an interim stable matching.  %Note that under the stylized assumption, all agents have at most $k$ interviews.  

The PI has written on the communicating requirements for achieve a stable matching under a similar utility model but when agents know their  actual utilities \cite{ashlagi2020clearing}. The key difference is that in the interview match we assume no restriction on the communication of a-priori preferences but rather attempt to limit the number of interviews after eliciting those preferences. In \cite{ashlagi2020clearing}, when the market has a tier structure, agents in each tier signal to a target tier from which they can guarantee to match; we believe  that a similar analogue of safety-interviews should arise in the interview match. The problem is more challenging when the tiers are soft and agents may only probabilistically prefer higher to lower tiers (see  \cite{DBLP:conf/innovations/AshlagiBSTZ21} for recent work by the PIs on typical outcomes in such markets when agent know their preferences).


